mu-complete Suslin trees on mu^+

We prove that mu = mu^{< mu}, 2^mu = mu^+ and ``there is a non reflecting stationary subset of mu^+ composed of ordinals of cofinality < mu'' imply that there is a mu-complete Souslin tree on mu^+ .

==> mssymb.tex <==

\message{Not using the real mssymb file}
\message{Inputting amssym.def and amssym.tex instead}
 {\catcode`\@11 \global\def\setboxz@h{\setbox0\hbox}
	\global\def\wdz@{\wd0 }
 }

\input amssym.def
\input amssym.tex
\def\napprox{\not\approx}

